Adaptable and Verifiable BDI Reasoning

Long-term autonomy requires autonomous systems to adapt as their capabilities no longer perform as expected. To achieve this, a system must first be capable of detecting such changes. In this position paper, we describe a system architecture for BDI autonomous agents capable of adapting to changes in a dynamic environment and outline the required research. Specifically, we describe an agent-maintained self-model with accompanying theories of durative actions and learning new action descriptions in BDI systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{117}
\providecommand{\publicationstatus}{R.C. Cardoso, A. Ferrando, D. Briola, C. Menghi,\\ T. Ahlbrecht (Eds.): First Workshop on Agents and\\ Robots for reliable Engineered Autonomy 2020 (AREA'20).\\
EPTCS 319, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.319.9}{10.4204/EPTCS.319.9}}
\pdfoutput=1

